AViTMP: A Tracking-Specific Transformer for Single-Branch Visual Tracking

Visual object tracking is a fundamental component of transportation systems, especially for intelligent driving. Despite achieving state-of-the-art performance in visual tracking, recent single-branch trackers tend to overlook the weak prior assumptions associated with the Vision Transformer (ViT) encoder and inference pipeline in visual tracking. Moreover, the effectiveness of discriminative trackers remains constrained due to the adoption of the dual-branch pipeline. To tackle the inferior effectiveness of vanilla ViT, we propose an Adaptive ViT Model Prediction tracker (AViTMP) to design a customised tracking method. This method bridges the single-branch network with discriminative models for the first time. Specifically, in the proposed encoder AViT encoder, we introduce a tracking-tailored Adaptor module for vanilla ViT and a joint target state embedding to enrich the target-prior embedding paradigm. Then, we combine the AViT encoder with a discriminative transformer-specific model predictor to predict the accurate location. Furthermore, to mitigate the limitations of conventional inference practice, we present a novel inference pipeline called CycleTrack, which bolsters the tracking robustness in the presence of distractors via bidirectional cycle tracking verification. In the experiments, we evaluated AViTMP on eight tracking benchmarks for a comprehensive assessment, including LaSOT, LaSOTExtSub, AVisT, etc. The experimental results unequivocally establish that, under fair comparison, AViTMP achieves state-of-the-art performance, especially in terms of long-term tracking and robustness. The source code will be released at https://github.com/Tchuanm/AViTMP.

==> tables/attention.tex <==
\begin{table}[t]
	\centering
 	\caption{ Comparison of different attention and decoder components.
	}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\dist}{\hspace{14pt}}%
	\newcommand{\yes}{\textcolor{black}{\checkmark}}
	% \resizebox{1.\columnwidth}{!}{%
        \begin{tabular}{c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        	\toprule
        	        Attention  & LaSOT         & LaSOTExtSub\\
        	\midrule
                 + Plain Attention    & xxx   & xxx \\
                    % + Sparse  Attention   & \scnd{xxx}  & xxx \\  %22
                    +Zero-centered Attention   & \best{xxx}  & xxx          \\
        + Plain Decoder    & \best{xxx}  & xxx               \\
        + Dense-Fused Decoder    & \best{xxx}  & xxx               \\
        \bottomrule
        \end{tabular}
	% }
	\label{tab:attention}%
\end{table}



==> tables/lasot_attributes_figures.tex <==
\begin{figure*}[t]
\centering
\subfloat[Illumination  Variation.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/IV.pdf}}
  \hfill
\subfloat[Partial Occlusion.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/POC.pdf}}
    \hfill
  % \begin{subfigure}{0.2454\linewidth}  
  %   \includegraphics[width=\columnwidth, keepaspectratio]{figures/LaSOT_attributes/DEF.pdf}} 
  %   \caption{Deformation.}  \vspace{-1mm}
  %  
  %     \hfill
  % \begin{subfigure}{0.2454\linewidth}  
  %   \includegraphics[width=\columnwidth, keepaspectratio]{figures/LaSOT_attributes/MB.pdf}} 
  %   \caption{Motion Blur.}  \vspace{-1mm}
  %  
  % \hfill
\subfloat[Camera Motion.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/CM.pdf}}
    \hfill   
\subfloat[Rotation.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/ROT.pdf}} 
      \hfill  \\
\subfloat[Background Clutter.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/BC.pdf}} 
      \hfill
\subfloat[Viewpoint Change.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/VC.pdf}}
  \hfill  
\subfloat[Scale Variation.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/SV.pdf}}
    \hfill
\subfloat[Full Occlusion.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/FOC.pdf}} 
      \hfill     \\
\subfloat[Fast Motion.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/FM.pdf}} 
      \hfill   
\subfloat[Out-of-view.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/OV.pdf}}
  \hfill
\subfloat[Low Resolution.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/LR.pdf}}
    \hfill 
\subfloat[Aspect Ratio Change.]{\includegraphics[width=0.245\linewidth]{figures/LaSOT_attributes/ARC.pdf}}
    % \vspace{-0mm}
    \caption{Attributes success rate visualization comparison of state-of-the-art methods on LaSOT~\cite{lasot} benchmark.  
}
\label{lasot_attributes_fig}
% \vspace{-0mm}
\end{figure*}

==> tables/nfs.tex <==
\begin{table}[!t]
	\centering
	\caption{Comparison with the state-of-the-art methods on NFS30~\cite{Galoogahi_2017_ICCV_NFS}.
	}  
	% \vspace{-0mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\dist}{\hspace{5pt}}%
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        	\toprule
        	    & \textbf{}  &   &SeqTrack  & Keep   & OSTrack  &     &STARK &STARK &  Tr  & Super  & Pr        & Siam           \\
        	     & \textbf{Ours}  & GRM       &B256 &Track   &256    &TransT  &ST50  &ST101 & DiMP     & DiMP   & DiMP    & R-CNN \\
        	    &  &\cite{gao2023GRM}         &\cite{chen2023seqtrack}  &\cite{keeptrack}   &\cite{ye2022OSTrack}  &\cite{chen2021transt}  &\cite{stark} &\cite{stark} &\cite{trdimp}  & \cite{Danelljan_2019_github_pytracking} & \cite{prdimp}  & \cite{siamr-cnn}  \\          
        	\midrule
        	% UAV123  &\best{70.1}  &69.2 &\scnd{69.7}  &68.3     &69.1    &69.1 &68.2 &67.5   & 67.7   & 68.0 & 64.7        & 57.4 & 64.9  & -   & 65.3 \\
                % TNL2k   &\scnd{54.5}    &\best{54.9}  &-    &54.3  &50.7   &-    &-  &-       &49.2       &47.0     &38.4            &-     &52.3      &44.9     & 44.7           \\ 
                NFS30     &66.3  &65.6   &\best{67.6}   &66.4  &64.7 &65.7  &65.2  &66.2 &\scnd{66.5}     & 64.8   & 63.5 & 63.9          \\
         \bottomrule

        \end{tabular}
	}  
	\label{tab:nfs}%
\end{table}




==> tables/otb.tex <==
\begin{table}[!t]
	\centering
	\caption{Comparison with state-of-the-art on the OTB100~\cite{WU_2015_TPAMI_OTB}.}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\dist}{\hspace{5pt}}%
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        	\toprule
        	     &   & AiA & ToMP  & Keep  & STARK & Tr   &           & STARK & Super       & Pr         & Siam  & STM      \\
        	  &\textbf{Ours}       & Track & 101   & Track & ST101 & DiMP & TransT & ST50  & DiMP        & DiMP       & R-CNN & Track   \\
        	  &     &\cite{gao2022aiatrack}  &\cite{tomp}  & \cite{keeptrack} & \cite{stark} &\cite{trdimp} & \cite{chen2021transt}   & \cite{stark} &\cite{Danelljan_2019_github_pytracking} & \cite{prdimp} & \cite{siamr-cnn} & \cite{fu2021stmtrack}  \\
        	\midrule
        	AUC  &70.3        & 69.6  & 70.1       & 70.9        & 68.1 & 71.1 & 69.4        & \scnd{71.4} & 70.1 & 69.6 & 70.1 & \best{71.9} \\
        	\bottomrule
        \end{tabular}
	}
	\label{tab:otb}%
\end{table}


==> tables/scale-change-ablation.tex <==
\begin{table}[t]
	\centering
	\caption{The size change threshold of training frames update method during inference.
	} 
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\dist}{\hspace{14pt}}%
	\newcommand{\yes}{\textcolor{black}{\checkmark}}
	\resizebox{1\linewidth}{!}{%
        \begin{tabular}{c@{\dist}|c@{\dist}|c@{\dist}|c@{\dist}|c@{\dist}}
        	\toprule
        	        Size (H$\times$W)  &$>$4 or $<\frac{1}{4}$      &$>$9 or $<\frac{1}{9}$     &$>$16 or $<\frac{1}{16}$     &$>$25 or $<\frac{1}{25}$    \\
        	\midrule
                 LaSOT    & 69.8   &70.3  & 70.7   & 70.1 \\               
        \bottomrule
        \end{tabular}
	}
	\label{tab:scale-change}%
\end{table}


